CAPGrasp: An $\mathbb{R}^3\times \text{SO(2)-equivariant}$ Continuous Approach-Constrained Generative Grasp Sampler

We propose CAPGrasp, an $\mathbb{R}^3\times \text{SO(2)-equivariant}$ 6-DoF continuous approach-constrained generative grasp sampler. It includes a novel learning strategy for training CAPGrasp that eliminates the need to curate massive conditionally labeled datasets and a constrained grasp refinement technique that improves grasp poses while respecting the grasp approach directional constraints. The experimental results demonstrate that CAPGrasp is more than three times as sample efficient as unconstrained grasp samplers while achieving up to 38% grasp success rate improvement. CAPGrasp also achieves 4-10% higher grasp success rates than constrained but noncontinuous grasp samplers. Overall, CAPGrasp is a sample-efficient solution when grasps must originate from specific directions, such as grasping in confined spaces.

==> tex/Sections/7_limitations.tex <==
\section{Limitations}

Our work has two apparent limitations, both stemming from the constraints. The first limitation is that $\matr{A}$ is selected manually or through some simple-to-compute geometrical features. For instance, in the shelf-picking task, we manually set $\Vec{v}_A$ and $\alpha$ such that the generated grasps would have a low chance of colliding with the environment. The second limitation is that we cannot pose non-isotropic approach constraints like elliptical ones.

==> tex/Sections/acknowledgment.tex <==
\section*{ACKNOWLEDGMENT}

We would like to show our gratitude to the Swedish Research Council, Knut and Alice Wallenberg Foundation, and Horizon2020 ERC BIRD.
